Trollthrottle -- Raising the Cost of Astroturfing

Astroturfing, i.e., the fabrication of public discourse by private or state-controlled sponsors via the creation of fake online accounts, has become incredibly widespread in recent years. It gives a disproportionally strong voice to wealthy and technology-savvy actors, permits targeted attacks on public forums and could in the long run harm the trust users have in the internet as a communication platform. Countering these efforts without deanonymising the participants has not yet proven effective; however, we can raise the cost of astroturfing. Following the principle `one person, one voice', we introduce Trollthrottle, a protocol that limits the number of comments a single person can post on participating websites. Using direct anonymous attestation and a public ledger, the user is free to choose any nickname, but the number of comments is aggregated over all posts on all websites, no matter which nickname was used. We demonstrate the deployability of Trollthrottle by retrofitting it to the popular news aggregator website Reddit and by evaluating the cost of deployment for the scenario of a national newspaper (168k comments per day), an international newspaper (268k c/d) and Reddit itself (4.9M c/d).

==> bibcleanup.tex <==
\AtEveryBibitem{% Clean up the bibtex rather than editing it
 \clearlist{address}
 \clearfield{date}
 \clearfield{eprint}
 \clearfield{isbn}
 \clearfield{issn}
 \clearlist{location}
 \clearfield{month}
 \ifentrytype{book}{
  \clearname{editor}
  }{}
\ifentrytype{inproceedings}{
  \clearname{editor}
  \clearfield{volume}
  \clearfield{url}
}{}
\ifentrytype{incollection}{
  \clearname{editor}
  \clearfield{volume}
  \clearfield{url}
}{}
\ifentrytype{proceedings}{
 \clearname{editor}
 \clearfield{volume}
 \clearfield{url}
}{}
\ifentrytype{article}{
 \clearfield{url}
 % \clearlist{publisher}
 % \clearfield{series}
 % \clearfield{volume}
}{}
}




==> implement.tex <==

\section{Implementation Details}\label{sec:implement}

We translated the
Multiprecision Integer and Rational Arithmetic Cryptographic Library
(MIRACL) from C to JavaScript using emscripten and some manual
modifications for portability. 
%
As this library is widely used to implement elliptic curve
cryptography and large integers, this translation could be of independent
interest \cite{MIRACLjs}.
%%%%%%%%%%%%%%%%%%55
%%%%%%%%%%%%%%%%%%%%5
%\footnote{Available at \url{http://upload.preliminary.bplaced.net/trollthrottle_dev.zip}.}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
We use this library to implement Brickell and Li's pairing based DAA 
scheme using Barreto-Naehrig (BN)~\cite{BN-pairing} 
elliptic curve at the 128-bit security level.
%
Furthermore, we use
libsodium~\cite{libsodium}
for 
digital signatures used in the identity verification protocol (based on Ed25519 with 256 bit keys),
hashing (BLAKE2B),
authenticated public-key encryption 
(based on XSalsa20 stream cipher and X25519 key exchange with 256 bit keys)
and
randomness generation.
%
For key derivation, we used PBKDF2 in Crypto-js~\cite{crypto-js} with
100\,100 iterations.\footnote{Default for server-side
storage of passwords in LastPass~\cite{lastpass-iterations}.}

==> lstsettings-sapic.tex <==
\lstdefinelanguage{sapic}{
  morekeywords=[1]{
    %%% KEYWORDS
	out, in, if, then, else, event, insert, delete, lookup, as, in, lock, unlock, let,
        theory, begin, builtins, functions, equations, +, lemma,
        exists-trace
    },
  sensitive=true,
  morecomment=[l]{\#},
  morecomment=[l]{//},
  morestring=[b]',
  morestring=[s]{`}{'},
  % morestring=[s]{[}{]},
}

\lstdefinestyle{sapic}{
    language={sapic}, 
	stringstyle=\rm\textup,
	keywordstyle=[1]\sf,
 	keywordstyle=[2]\rm\upshape,
	literate={||}{{$\mid$}}1
	{new}{{$\nu$}}1
	{==>}{{$\implies$}}2
        {Ex}{{$\exists$}}1
        {All}{{$\forall$}}1
        {\&}{{$\land$}}1
	{<}{{$\langle$}}1
	{>}{{$\rangle$}}1
	{\#}{{}}0
	{(}{{$($}}1
	{)}{{$)$}}1
	{:=}{{$\defeq$}}2
}


\lstset{style=sapic,
	mathescape=true, 
	commentstyle=\rm\itshape,
	showstringspaces=false,
    frameround=ftff,
    % frame=single,
	captionpos=b,
	columns=flexible,
escapeinside={(*}{*)},
basicstyle=\it\small,	
% escapechar=!,
tabsize=2,
breaklines=true,
showstringspaces=true,
emph={label}
} 

% vim: ft=tex


==> sec-proof-account-tracking-registration.tex <==
\subsubsection{Tracking registrations}

A very rudimentary form of accountability can be used to detect
a large number of sock puppets generated by an issuer that colludes
with a verifier to produce an unreasonably large number of users.
E.g., in the subscription model, the approximate maximum number of
users is public knowledge.

\begin{definition}\label{def:acctrack}
We say that the system's accountability mechanism 
tracks registrations
if
for every adversary $\A$, every $\secparam$, the probability
$\Pr[\ExpAcctrack(\secparam)=1]$ is negligible $\secparam$.

\begin{center}
\begin{figure}[H]
    \begin{experiment}{\ExpAcctrack(\secparam)}
    \flushleft
$\CU \leftarrow \emptyset$; $\HU \leftarrow \emptyset$; $V \leftarrow \emptyset$;   \\
$\USK \leftarrow \emptyset$; $\COMM \leftarrow \emptyset$; $\ver \leftarrow \emptyset$;  \\
$(\sk_\iss,\pk_\iss) \rexec \Setup(\secparam)$ \\\
$\Or = \{ \CorruptU(\cdot), \CorruptV(\cdot,\ver), \CUser(\cdot,\ver,\sk_\iss),$ \\
$\CComment(\cdot,\cdot,\cdot,\pk_\iss), \UserJoin(\cdot,\ver,\sk_\iss)\}$\\
run $V \rexec \A^{\Or}(\crs,\pk_\iss)$\\
$\GB_s = \{ \gb \in \GB : \Attribute(\gb)=V \}$\\
$\USK_s = \{ (\uid,\sk_{\uid},\cred_{\uid},V') \in \USK : V'=V \}$\\
$V_s = \{ (V',\uid) \in \VM : V'=V \}$\\
Return $1$ if $|\GB_s|\neq|\USK_s|+|V_s|$ and $\forall\uid$ s.t.\\
$\exists (\cdot, \uid) \in V_s \vee$ 
$(\uid,\cdot,\cdot,\cdot)\in\USK_s$, the adversary has a valid pair\\
$(\sk_{\uid},\cred_{\uid})$
\end{experiment}
\caption{}
\end{figure}
\end{center}

%\begin{center}
%\begin{figure}[H]
%    \begin{experiment}{\ExpAcctrack(\secparam)}
%\indskip $\CU \leftarrow \emptyset$; $\HU \leftarrow \emptyset$; $V \leftarrow \emptyset$;   \\
%\indskip $\USK \leftarrow \emptyset$; $\COMM \leftarrow \emptyset$; $\ver \leftarrow \emptyset$;  \\
%\indskip $(\sk_\iss,\pk_\iss) \rexec \Setup(\secparam)$ \\\
%\indskip $\Or = \{ \CorruptU(\cdot), \CorruptV(\cdot,\ver), \CUser(\cdot,\ver,\sk_\iss),$ \\
%\indskip\indskip\indskip $\CComment(\cdot,\cdot,\cdot,\pk_\iss), \UserJoin(\cdot,\ver,\sk_\iss)\}$\\
%\indskip run $V \rexec \A^{\Or}(\crs,\pk_\iss)$\\
%\indskip $\GB_s = \{ \gb \in \GB : \Attribute(\gb)=V \}$\\
%\indskip $\USK_s = \{ (\uid,\sk_{\uid},\cred_{\uid},V') \in \USK : V'=V \}$\\
%\indskip $V_s = \{ (V',\uid) \in \VM : V'=V \}$\\
%\indskip Return $1$ if $|\GB_s|\neq|\USK_s|+|V_s|$ and $\forall\uid$ s.t.\\
%\indskip $\exists (\cdot, \uid) \in V_s \vee$ 
%\indskip$(\uid,\cdot,\cdot,\cdot)\in\USK_s$, the adversary has a valid pair\\
%\indskip $(\sk_{\uid},\cred_{\uid})$
%\end{experiment}
%\caption{}
%\end{figure}
%\end{center}
\end{definition}

\begin{theorem}[Tracking registrations]\label{thm:regtrack-p}
    The \trollthrottle protocol (see
    Def.~\ref{def:trollthrottle})
    satisfies Registration tracking (see Def.~\ref{def:trolling}),
    if the underlying DAA scheme provides user-controlled traceability
    (Def.~\ref{def:user-controlled-traceability}).
\end{theorem}
\begin{proof}
 Assume there exists a PPT adversary A that can win the registration
    tracking game with non-negligible probability.
    W.l.o.g., assume that $A$ queries
\begin{itemize}
    \item $\CorruptV(\uid_i,\ver)$ and $\UserJoin(\uid_i, \ver, \sk_\iss)$ for $ i\in [1,p]$
    \item $\CUser(\uid_j,\ver, \sk_\iss)$ and $\CorruptU(\uid_j)$ for $ j \in [1,q]$
\end{itemize}
    for $p$,$q$ polynomial in $\secparam$, in order to receive
    $p+q$ pairs of credentials for fake users $(\cred_\uid,\sk^\DAA_\uid)$.

By definition of $\CUser$ and $\UserJoin$,
    $|\GB_s|= p+q$, 
    $|\USK_s|=q $,
    $|\USK_s|=p$ 
    and therefore $|\GB_s| =|V_s|+|\USK_s|$.
    %
The adversary can thus win in two cases:
    \emph{Case 1:} if $|\GB_s|>|V_s|+|\USK_s|$,
    \emph{case 2:} if $|\GB_s|<|V_s|+|\USK_s|$.

\emph{Consider case 1:} There exists a genesis tuple in $\GB_s$ that
    was not created during $A$'s oracle queries, i.e., that does not
    correspond to some $\uid$ s.t. 
    $\exists(\cdot, \uid)\in V_s$ 
    or
    $\exists (\uid,\cdot,\cdot,\cdot) \in \USK_s$.
    %
    Hence, $\A$ was
    able to forge a genesis tuple.
    %
    By definition of $\Comment$,
    every genesis tuple contains $\sig(\sk_V,h(1)^{\sk_\uid})$, a digital signature of the verifier.
    %
    If $A$ can win the registration tracking game with non-negligible probability,
    we can
    construct a PPT adversary $\A'$
    that can construct forgeries against the
    underlying digital signature scheme as follows:
    %
    $A'$ runs $\Setup_{\DAA}(\secparam)$and receives $(\pk_{I,\DAA},\sk_{I,\DAA})$. 
    Obtaining the issuer's private key, $\A'$ can execute all \trollthrottle algorithms
    in Def.~\ref{def:trollthrottle}, except the $\JoinIssue$
    protocol as this requires the calculation of a digital signature.
    %
    By modifying the $\JoinIssue$ protocol to query the signature oracle
    instead of computing the signature, $\A'$ can perfectly simulate
    the oracles in $\ExpAcctrack$ and output 
    the second and third component of $\gb$ to produce a forgery.
    
\emph{Consider case 2:} $\A$ produced a valid pair
    $(\sk_{\uid},\cred_{\uid})$, that does not correspond to some
    $\gb\in \GB_s$, i.e., $\A$ was able to obtain credential and secret
    key for some $\uid$ without running $\CorruptU$ or $\UserJoin$ on
    $\uid$, as this would have created a genesis tuple. 
    %
    Given $\A$,
    we can construct a PPT adversary $\A'$ against user-controlled traceability,
    again following simulation steps~\ref{it:oracle-sim} as in
    Theorem~\ref{thm:trolling-p}.

    $\A'$ obtains $(\sk_{\uid},\cred_{\uid}) \rexec \A^{\Or}(\crs,\sk_\iss)$
(for $\Or$ as above) 
and computes $\sigma=\Sign_\DAA(\sk_{\uid},\cred_{\uid},m,\dom)$ 
for some arbitrary message $m$ and basename $\dom$ not queries before.
%
$A'$ returns $\mathvalue{out}=(\uid,\sigma,m,\dom)$
and thus wins the user-controlled traceability experiment with 
non-negligible probability.

Whenever $A$ wins, she is either in case 1 or case 2, hence either or
both cases occur with non-negligible probability, thus contradicting
the assumptions on the digital signature scheme and the DAA scheme.
\end{proof}


==> sec-proof-unforgeability.tex <==
\subsection{Unforgeability}

\begin{definition}\label{def:unforge}
We say that the system is unforgeable if
for every adversary $\A$, every $\secparam$, the probability
$\Pr[\ExpUnf(\secparam)=1]$ is negligible $\secparam$.

\begin{figure}[H]
\begin{experiment}{\ExpUnf(\secparam)}
\flushleft
$\CU \leftarrow \emptyset$; $\HU \leftarrow \emptyset$; $V \leftarrow \emptyset$;   \\
$\USK \leftarrow \emptyset$; $COMM \leftarrow \emptyset$; $\ver \leftarrow \emptyset$;  \\
$(\sk_\iss,\pk_\iss) \rexec \Setup(\secparam)$ \\
$\Or = \{ \CorruptU(\cdot), \CorruptV(\cdot,\ver), \CUser(\cdot,\ver,\sk_\iss),$ \\
$\CComment(\cdot,\cdot,\cdot,\pk_\iss), \UserJoin(\cdot,\ver,\sk_\iss)\}$\\
$(\nym^*,\dom^*,m^*,\comm^*) \rexec \A^{\Or}(\crs,\pk_\iss)$\\
Return $0$ if $\Verify(\pk_\iss,\nym^*,\dom^*,m^*,\comm^*)=0$\\
Return $1$ if:\\
1) there exists no tuple $(\cdot,\nym^*, \dom^*, m^*, \cdot)$ in $COMM$, and\\
2) $\forall_{\uid^* \in \HU \cup \CU}$ $\nym^* \not= \NymGen(\sk_{\uid^*},\dom^*)$\\
\end{experiment}
\caption{}
\end{figure}

%\begin{figure}[H]
%\begin{experiment}{\ExpUnf(\secparam)}
%\indskip $\CU \leftarrow \emptyset$; $\HU \leftarrow \emptyset$; $V \leftarrow \emptyset$;   \\
%\indskip $\USK \leftarrow \emptyset$; $COMM \leftarrow \emptyset$; $\ver \leftarrow \emptyset$;  \\
%\indskip $(\sk_\iss,\pk_\iss) \rexec \Setup(\secparam)$ \\
%\indskip $\Or = \{ \CorruptU(\cdot), \CorruptV(\cdot,\ver), \CUser(\cdot,\ver,\sk_\iss),$ \\
% \indskip\indskip\indskip $\CComment(\cdot,\cdot,\cdot,\pk_\iss), \UserJoin(\cdot,\ver,\sk_\iss)\}$\\
% \indskip $(\nym^*,\dom^*,m^*,\comm^*) \rexec \A^{\Or}(\crs,\pk_\iss)$\\
% \indskip Return $0$ if $\Verify(\pk_\iss,\nym^*,\dom^*,m^*,\comm^*)=0$\\
%\indskip Return $1$ if:\\
%\indskip\indskip 1) there exists no tuple $(\cdot,\nym^*, \dom^*, m^*, \cdot)$ in $COMM$, and\\
%\indskip\indskip 2) $\forall_{\uid^* \in \HU \cup \CU}$ $\nym^* \not= \NymGen(\sk_{\uid^*},\dom^*)$\\
%\end{experiment}
%\caption{}
%\end{figure}

\end{definition}

%{\color{red} Lucjan's comment: \color{blue}we have to discuss if non-frameability should address a malicious issuer.
%If not then it can be merged with non-frameability. The current definition also assumes that the $\JoinIssue$ protocol
%is executed honestly by the issuer (otherwise we would have to introduce a new oracle) - discuss.}
%
%{\color{red} Robert's comment: \color{blue} I'll also note that
%condition 2) implies condition 1) because \NymGen is deterministic and
%all comments in COMM are created using \Comment.}

\begin{theorem}[Unforgeability]\label{thm:unforge-p}
    The \trollthrottle protocol (see
    Def.~\ref{def:trollthrottle})
    satisfies Unforgeability (see Def.~\ref{def:trolling})
    if the underlying DAA scheme provides user-controlled traceability
    (Def.~\ref{def:user-controlled-traceability}) and is instantly linkable.
\end{theorem}
\begin{proof}
Assume there exists a PPT adversary $\A$ that can win the unforgeablity game with non-negligible probability.
Then, for the returned $(\nym^*, \dom^*, m^*,\allowbreak \comm^*)$ such that
$\Verify(\pk_\iss,\nym^*,\dom^*,m^*,\comm^*)=1$,
$(\cdot,\nym^*, \dom^*, \allowbreak m^*, \cdot)\not\in \COMM$,
it holds that
$\forall \uid^* \in \HU \cup \CU \; \nym^* \neq \NymGen(\sk_{\uid^*},\dom^*)$.
We will now show how to construct a PPT adversary $\R$ against the user-controlled traceability. 
The reduction $\R$ simulates the oracles according to ~\ref{it:oracle-sim}.

%\paragraph{Initialisation}:\label{it:oracle-sim-init}
%$\UID, \HU, \CU, \USK, \VM, \GB, \COMM, \ver \leftarrow \emptyset$ are global sets, $(\sk_V,\pk_V))\rexec \kgsign(\secparam)$

%
%\paragraph{Oracle Simulation}:\label{it:oracle-sim}
%$\R$ can run the following oracle queries according to ~\cite{DBLP:journals/iacr/BrickellL10}
%\begin{itemize}
%\item $\Sign_\DAA(S,\dom,m)$\\ On input of a signer's identity S, a basename $\dom$ (either $\bot$ or a data string), a message m the oracle returns signature $\sigma$.
%\item $\Join_\DAA(S)$
%    On input of a signer's identity $S$ of her choice, the adversary obtains credentials $\cred$. The secret key $\sk$ is kept secret.
%    
%\item $\CorruptU_\DAA(S)$
%   On input of a signer's identity $S$, the value $\sk$ is returned to the adversary
%\end{itemize}
%
%Using those oracle the reduction $\R$ simulates the TrollThrottle oracles as follows:
%\UID replaces the origial \USK set and only contains the \uids and respective credentials and the secret keys $\sk_{\uid }'$ that A used to generate the genesis tuples.
%\\Those "fake" secret keys are independent of the secret keys that Join generates and which correspond to the credentials
%\begin{itemize}
%
%\item $\CorruptU(\uid)$
%
%If $(\uid,\cdot,\cdot)\not\in \USK$, $\R$ returns $\perp$,  else $\R$
%        obtains $\cred_{\uid}$ from a lookup in $\USK$.
%$\R$ sets $\sk_{\uid}=\CorruptU_{\DAA}(\uid)$, 
%        $\CU = \CU \cup \set{\uid}$,$\HU = \HU\setminus \set{\uid}$
%        and returns $(\cred_{\uid},\sk_{\uid})$.
%\\Wlog we not allow $\CorruptU$ queries after $\CComment$ queries. Any adversary can obtain 
%the same results by first running $\CorruptU$ and calculating comments afterwards by executing 
%$\Comment(\pk_\iss,\sk_{\uid},\cred_{\uid},\cdot,\cdot)$ with the obtained secret key $\sk_{\uid}$.
%\\A' checks if \uid is in \UID an outputs $\perp$ if not. It queries Corrupt on the respective \uid, receives the respecive secret key $\sk_{\uid}$, puts it into \CU and returns ($creds_{\uid}$, $\sk_{\uid}$)   
%
%\item $\CorruptV(\uid,\ver,V)$
%
% sets $\ver[V,\uid]=1$ and $\VM=\VM \cup\{ (V,\uid)\}$
%
%\item $\CUser(\uid,\ver,\sk_\iss,V)$
%if \uid $\in (\HU \cup \CU)$ $\R$ returns $\perp$ else $\R$ sets 
%\begin{itemize}
%\item $\ver[V,\uid]=1$
%\item executes internally the $\Join_{\DAA}$ protocol receiving $(\sk'_{\uid}, \cred_{\uid})$
%\item $\sk'_{\uid} \rexec \{0,1\}^*$ uniformly at random
%\item $\nym^1_{\uid} = \NymGen(\sk'_{\uid},1)$
%\item $\gb_{\uid}= (\pk_V, \nym^1_{\uid}, \sig(\sk_V, \nym^1_{\uid})$
%\item $\USK = \USK\cup \{(\uid,\sk'_{\uid},\cred_{\uid})\}$, $\GB = \GB\cup \set{\gb_{\uid}}$, $\HU \setminus \{\uid\}$
%\end{itemize}
%\\A' first checks if \uid $\in$ \HU or \CU and returns $\bot$ if so. Else it sets ver[V,\uid]=1 and calls Join in order to receive the credentials.
%A creates the genesis tuple as follows:
%\\A chooses $\sk_{\uid }'$ uniforlmy at random from the DAA keyspace $\kappa_{s,u}$ and computes the genesis tupe gb corresponding to $\sk_{\uid }'$. It puts ($\sk_{\uid }'$,$creds_{\uid}$,\uid) into \UID, \uid in \HU and gb into \GB
%
%\item $\UserJoin(\uid,\ver,\sk_\iss,V)$
%\\If $\uid \in (\HU \cup \CU) \vee \ver[V,\uid]=1$, $\R$ returns $\perp$, 
%\\else $\R$ sets
%\begin{itemize}
%\item executes $(\sk'_{\uid},\cred_{\uid}) \rexec \Join_{\DAA}(\pk_\iss)$
%\item $\sk'_{\uid} \rexec \{0,1\}^*$ uniformly at random
%\item $\nym^1_{\uid} = \NymGen(\sk'_{\uid},1)$
%\item $\gb_{\uid}= (\pk_V, \nym^1_{\uid}, \sig(\sk_V, \nym^1_{\uid})$
%\item $\USK \gets \USK \cup \{(\uid,\sk'_{\uid},\cred_{\uid})\}$,
%    $\GB \gets \GB \cup \{\gb_{\uid}\}$,
%        $\HU \gets \HU \setminus \{\uid\}$
%\end{itemize}
%
%\item $\CComment(\uid,\dom,m,\pk_\iss)$
%if \uid $\not\in \HU$ $\R$ returns  $\perp$ else $\R$:
%\begin{itemize}
%\item $n \rexec \{0,1\}^\lambda$
%\item finds tuple $(\uid,\sk_{\uid},\cred_{\uid}) \in \USK$
%\item $\sigma= \Sign_{\DAA}(\sk_{\uid},\cred_{\uid},m,\dom)$
%\item $\nym= \NymExtract(\sigma)$
%\item $\Pi = \perp$ for the basic protocol version and $\CreateProof(\pk_{\iss},\sk_{\uid},\GB)$ for the extended protocol version
%\item $\comm=(\sigma,\Pi, \nym, \dom, m)$
%\item $\COMM \gets \COMM \cup\{ (\uid,\nym,\dom,m,\comm)\}$
%\end{itemize}
%and returns $(\comm,\nym)$
%\\On input \uid, dom, m and the issuer's pblic key, A' calls Sign on signer's identity \uid, basename dom and message m to obtain the signature $\sigma$
%Then, A' creates the commit as comm=($\sigma$, $\Pi$), 
%\\with $\Pi=\perp$ for the basic protocol and CreateProof($\sk_{DAA}', \GB$) for the exteded protocol version, i.e. A runs GetProof() on its own with the "fake" secret key $\sk_{\uid }'$
%Furthermore A' computes nym= NymExtract($\sigma$) and returns (nym,comm)
%
%\end{itemize}

With non-negligible probability, $\R$ obtains $(\nym^*,\dom^*,m^*,\comm^*) \rexec \A^{\Or}(\crs,\pk_\iss)$
for 
$\Or = \{ \CorruptU(\cdot), \CorruptV(\cdot,\ver), \CUser(\cdot,\ver,\allowbreak \sk_\iss),$
$\CComment(\cdot,\cdot,\cdot,\pk_\iss), \UserJoin(\cdot,\ver,\sk_\iss)\}$

Let us denote $out=(\uid^*,\sigma^*,m^*,\dom^*)$, where $\comm^* = (\sigma^*, \nym^*,\Pi^*,m^*,\dom^*)$. 
Since we know that
 $\A$ only wins if $(\cdot,\nym^*, \dom^*, m^*, \cdot)\not\in \COMM$ is not a response to any signing query made by $\R$. What's more, because of the instant linkability we know that this signature does not correspond to
 any secret key of an existing user (corrupted or honest) and is valid even for the revocation list containing the
 secret keys of corrupted users. Therefore, by returning $out$ the reduction $\R$ wins and we have 
$$\Pr[\ExpUnf(\secparam)=1] = \Adv[\R^{trace}_{\DAA}] \leq \negl.$$

%\paragraph{We can construct} a probablistic polynomial time adversary A' against user-controlled-tracability by simulating A.
%A' simulates the oracles for $A$ as previously in the trolling experiment.  
%%(as described in the proof to Lemma~\ref{}),
%%%%%%%%%%%%%%%%%
%As defined in the oracle simulation, all Sign-queries must originate from \CComment-queryies, which add the signature to COMM.
%%and \CComment makes sure that T*O*D*O relation between $\nym^*$, $\dom^*$ and $m^*$ from 
%%T*O*D*O Is this still nessasary?

\end{proof}

